SEPAL: Towards a Large-scale Analysis of SEAndroid Policy Customization

To investigate the status quo of SEAndroid policy customization, we propose SEPAL, a universal tool to automatically retrieve and examine the customized policy rules. SEPAL applies the NLP technique and employs and trains a wide&deep model to quickly and precisely predict whether one rule is unregulated or not.Our evaluation shows SEPAL is effective, practical and scalable. We verify SEPAL outperforms the state of the art approach (i.e., EASEAndroid) by 15% accuracy rate on average. In our experiments, SEPAL successfully identifies 7,111 unregulated policy rules with a low false positive rate from 595,236 customized rules (extracted from 774 Android firmware images of 72 manufacturers). We further discover the policy customization problem is getting worse in newer Android versions (e.g., around 8% for Android 7 and nearly 20% for Android 9), even though more and more efforts are made. Then, we conduct a deep study and discuss why the unregulated rules are introduced and how they can compromise user devices. Last, we report some unregulated rules to seven vendors and so far four of them confirm our findings.

==> 6-rq1.tex <==
%!Tex root = ./sabre.tex
\subsection{RQ1: How does the policy customization evolve across Android versions?}

For each Android version, the percentage and number of manufacturers' unregulated rules are shown in Fig~\ref{fig:average cross version}. %It indicates that the manufacturers have realized the necessity of reducing the number of rules, but the quality of the rules has gradually drifted away from Google's criterion. \guozhu{It is the reason???}
Specifically, the evolution of policy customization has gone through three phases:
%--Figure---
\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth,height=4cm]{figures/average-cross_version.pdf}
    \caption{The average number of (unregulated) rules and occupied percentages per Android versions}
    \label{fig:average cross version}
    \vspace{-0.4cm}
\end{figure}


\textit{1) }In Android 5, Google just fully enforced SEAndroid in the system. The official policy is still lenient and coarse-grained. For most manufacturers, they didn't have to perform heavy customization on \emph{RRs}.
On average, each image contains 279 (5.13\%) unregulated atomic rules.
In fact, across 13 manufacturers in the dataset of Android 5, Samsung and Huawei are the major contributors (94.57\%) to the unregulated rules in Android 5. For other manufacturers, less than one hundred atomic rules are added. 
Due to the lack of limitations on app processes asserted by \emph{neverallow rules}, 20.20\% of the rules in Android 5 are defined by app-related domains. Most of them are explicitly forbidden in the later version of Android.
Besides that, a typical category of the unregulated rules in Android 5 is defined by coarse-grained attributes such as \emph{proc}, \emph{sysfs}, and \emph{unconfineddomain}. These rules respectively allow the subject to access nearly all the nodes in \textsfs{/proc}, \textsfs{/sys/fs} and any other mounted filesystems without a declared label. In the later versions of Android, Google defined many finer-grained types for the nodes in these filesystems and extremely limited access to proc and system partitions. 

\textit{2) }Since Android 6, Google gradually hardened the system by reducing the permissiveness of policy. Traditional coarse-grained types and attributes such as \emph{unconfineddomains} were abolished by Google, and the access to \textsfs{/proc} is strictly limited in Android 6.
%Yet our statistics show that the manufacturers are left behind. 
Though the average number of the customized atomic rules did not rise much (from 5442 to 5677),
the percentage of unregulated rules significantly increased from 5.13\% to 12.94\% in the 6.0 era. Manufacturers such as Samsung and Huawei didn't improve a lot in policy writing. In the meanwhile, ZTE, Meizu, and Oppo started to add more unregulated rules (nearly 20\%) at that time, resulting in the introduction of more coarse-grained attributes defined for data partition and device nodes in \textsfs{/dev}.
After that, in Android 7 some famous manufacturers were gradually aware of the security issues in the rules. They began to break down the coarse-grained attributes and types mentioned above, and remove the unnecessary rules related to app processes. The reason might be Google added more constrictions to lock down the application layer processes, leading to the decline in the unregulated rules from Android 6 to 7. The average number was reduced to 345 and the percentage was reduced to 7.83\%.


%Nevertheless, for most manufacturers, the customization on the policy has not been improved. 
%Some of them never update their rules. For instance, \emph{init}  process is allowed to reload policy at runtime since Android 4.3 via \textit{(allow init kernel:security load\_policy)}. This rule has been proven to be utilized to bypass SEAndroid in the wild. Thus the policy reloading mechanism has already been removed in the official policy of Android 6.0. However, it is still spotted in some Android 7 and Android 8 devices. 
%Another example shows that some manufacturers even remove the neverallow entries asserted by Google - the app processes are explicitly forbidden to access the \emph{video\_device}  character devices since Android 6.0. However, such allow patterns are still spotted in a Kaicom Android 8.1 device. From its CIL files, we find that the corresponding neverallow rule is removed by the policy writer, which may lead to a device node exposure attack. (See in \ref{subsection:Untrusted domains})

\textit{3) } In Android 8 and Android 9, the official policy has become much finer than ever before. 
%For instance, the number of rules in Android 9 is over 13 times that of Android 5.
However, the percentage of unregulated rules has risen again. The percentage came to 10.27\% in Android 8 and even rise to 19.68\% in Android 9,  which shows that the customization on the policy has not improved but become worse again. It has even become more and more difficult to keep up with the official policy for manufacturers. A reasonable explanation is the introduction of Project Treble~\cite{projecttreble}, which separates the lower-level customized code from the Android system framework.
 %\emph{RRs} have grown more strict~\cite{policycompatibility} — the number of neverallow entries has grown to 3550 in Android 9 with a nearly 50\% increment than that in Android 8. 
To update SEAndroid to work with Treble~\cite{projecttreble},  Manufacturers have to maintain their own hardware-specific policy rules and build their own images so that they can update those images independent of the AOSP, which is prone to introduce unregulated rules in the device. 
The vast bulk (27.61\%) of the unregulated rules defined for hardware abstraction layer (HAL) domains prove our concerns. These domains with a prefix \emph{hal} are assigned to the hardware layer processes implemented in vendor image since Android 8. %However, understanding the behaviors of these domains is truly difficult because the codes of these vendor-specific components are usually not public. 

\begin{comment}
\underline{\textbf{Findings: }} 
\textit{1)} The existence of unregulated rules is truly pervasive all over the versions.
\textit{2)} The percentage of the unregulated rules in manufacturers policy is growing over time, which shows manufacturers struggle to keep up with Google.
\kai{you may give more details. for example, changes of the subjects/objects in policies across different versions.}
\end{comment}

\begin{summary}
	As the AOSP continues to tighten policy rules, many unregulated rules that reside in the old versions of Android have disappeared in the latest version.
	However, new issues constantly emerges along with the increase of system complexity, resulting in an increase of the proportion of unregulated rules.
	 %However, new issues also arise as the version evolves, resulting in an increase in the proportion of unregulated rules.
\end{summary}

==> 6-rq2.tex <==
%!Tex root = ./sabre.tex
\subsection{RQ2: What is the difference in policy customization across different manufacturers?}

%The number of manufacturers-defined atomic rules can somehow reflect the degree of policy customization, and the percentage of unregulated rules reflect the quality of policy writing.
As aforementioned, manufacturers customize a varying number of policy rules as required.  
%Fig~\ref{fig:manufacturers case study} presents 12 manufacturers with the most number of customized rules. 
In this section, we select some manufacturers and investigate the unregulated rules residing in their devices. 
Through this analysis, we aim to unveil the status quo of unregulated rules among different manufacturers and infer the underlying reasons. Figure~\ref{fig:manufacturers case study} presents the distributions of unregulated rules of the two notable manufacturers:

%--Figure---
\begin{figure}[t]
\centering
  \subfigure[Distribution of Samsung's unregulated rules]{
  %\caption{Results of Similarity-based analyzer with Different Thresholds}
  \includegraphics[width=0.225\textwidth]{figures/samsung_casestudy2.pdf} 
  }
\hfill
  \subfigure[Distribution of Huawei's unregulated rules]{
  %\caption{Results of Similarity-based analyzer with Different Thresholds}
  \includegraphics[width=0.225\textwidth]{figures/huawei_casestudy2.pdf}
  }
%\hfill
%  \subfigure[Distribution of Xiaomi's unregulated rules]{
  %\caption{Results of Similarity-based analyzer with Different Thresholds}
%  \includegraphics[width=0.31\textwidth]{figures/xiaomi_casestudy2.pdf}
 % }
\caption{Distribution of notable manufacturers' unregulated rules. The high-low lines indicate the percentage range of corresponding samples}
\vspace{-0.5cm}
\label{fig:manufacturers case study}
\end{figure}
%---Figure Ends---


\noindent \textbf{Case study on Samsung. }
%heavy customization with lower unregulated rules 
Samsung is the only manufacturer that customizes policy heavily in Android 5 devices. 
On average, each image contains 1,203 unregulated rules in Android 5 and the number even comes to 3,268 in Android 6, which is several times that of other devices.% in the same period. 
%At that time, the average number of unregulated rules introduced in Samsung devices is over 2 thousand, while the number of most other manufacturers just reaches several hundred. 
It is most likely due to system developers were lack of policy writing expertise while doing heavy customization.
The evidence is that Samsung introduced many coarse-grained rules at the early stage. For instance, nearly half of the rules are related to the use of the socket. It could be caused by the overuse of common attributes, such as \emph{domain}, and \emph{unlabeled}, which leads to the introduction of many irrelevant atomic rules in one entry in the source code.
The situation has been improved since Android 7. The percentage of unregulated rules has been reduced to 7.89\% and the average number of unregulated atomic rules is only 500. 
It implies that Samsung realizes that it has introduced too many unnecessary rules, and deliberately shrunk these rules.
%Before Android 9, the percentage of unregulated rules in Samsung has remained at a low level.

Additionally, the policy customization of Samsung exhibits a unique feature - it defines rules in batches by introducing customized attributes. For example, \emph{newAttrs} are only introduced in Samsung devices. They play similar roles as \emph{base\_typeattrs} that introduced in the official CIL policy in Android 8. These attributes are responsible for a large number of unregulated rules of Samsung devices in Android 5 and 6.
Most of them were removed in Android 7 by Samsung, but several attributes such as \emph{platformappdomain} are still retained in the latest versions. It shows that Samsung has made its efforts in refining the policy rules in the early days.

\noindent\textbf{Case study on Huawei. }
%heavy customization with heavy unregulated rules
In Android 5, Huawei performs extremely well on policy customization - only 4.3\% of the atomic rules are classified as unregulated rules. 
Although Huawei does not perform as heavy policy customization as Samsung, the performance of Huawei is similar to that of Samsung in earlier Android versions. 
However, in Android 8, Huawei had little improvement and got difficult to keep up with the official policy evolution - 15.74\% of the atomic rules in Android 8 and 20.92\% of the atomic rules in Android 9 are classified as unregulated ones.
Among these rules, nearly 30\% of the unregulated rules introduced by Huawei in Android 8 are related to types that prefixed with \emph{hal}. All these types were newly added to refine the access control of the hardware abstraction layer (HAL) in official Android 8 due to the introduction of Project Treble. It suggests that Huawei's policy writers did not understand how to customize the hal-related rules in AOSP well. 
Further, we noticed that in some Huawei Android 8 devices, attribute \emph{domain} is allowed to read all the link files of the entrypoint executables in the system via ``\textsfs{allow domain exec\_type lnk\_file read}''. The combination of two coarse-grained attributes yields hundreds of unregulated atomic rules at one time. 
%\kai{the detailed analysis looks good.}

\begin{comment}
\noindent\textbf{Case study on Xiaomi. }
In Android 5, Xiaomi tried its best not to add unnecessary rules and kept the percentage of unregulated rules at a low level. On average, only 47 unregulated rules per image are introduced by Xiaomi.
After that, Xiaomi has 148 unregulated rules per images in Android 6, and 262 unregulated rules per image in Android 7.
Most of them are common issues about the coarse-grained file labels in \textsfs{/proc} and \textsfs{/sys}, or the overly permissive rules defined for app domains. 
After Android 8, just like what happens on Huawei, nearly 35\% of the hal-related unregulated rules are introduced, resulting in Xiaomi's percentage of unregulated rules increased significantly in Android 8 and 9.
\end{comment}
\noindent\textbf{Miscellaneous. }
Further, to study the overall ecosystem of policy customization across manufacturers, we analyze the images from 72 unique manufacturers under the same Android version (Android 8). Fig.~\ref{fig:manufacturers top10} presents the top 10 manufacturers with the highest unregulated percentage in Android 8. 
MTN is the manufacturers with the highest unregulated percentage (18.08\%) in Android 8. Note that the average unregulated percentage is only 10.64\% in Android 8.
To the best of our knowledge, the devices produced by these manufacturers are popular among some developing countries. 
However, their amount of unregulated per image is only two hundred, even lower than the average number (415) of Android 8.
Compared with the aforementioned notable manufacturers of the same Android version (shown in Fig~\ref{fig:manufacturers case study}), these manufacturers have some common features: they make as little customization as possible but have an extremely high percentage of unregulated rules. It shows that policy customization is an extremely hard task for these vendors. 
After looking into the unregulated rules spotted in these Android 8 images, we noticed that most of them are identical with the rules spotted in earlier versions of famous manufacturers' devices. For instance, they still use some coarse-grained attributes such as \emph{proc} and \emph{sysfs} in their hal-related rules. 

Furthermore, in Fig~\ref{fig:manufacturers case study}, some high-low lines indicate the differences between the phone models produced by the same manufacturers. We notice that the carrier may affect policy of the same model.
For instance, in Android 5, the policy of Samsung Note 3 for XAS (USA), a.k.a. N900P, is different from that of MCT (Canada), a.k.a. N900W. The unregulated percentage of the MCT is five percentage points higher than that of XAS. Specifically, the significant differences in their policy are related to the app process. It could happen when writing corresponding rules for pre-installed applications.

\begin{figure}[tb!]
    \centering
    \includegraphics[width=\linewidth,height=3.8cm]{figures/OEM_top10.pdf}
    \caption{Top 10 manufacturers with the highest percentage in Android 8}
    \label{fig:manufacturers top10}
    \vspace{-0.5cm}
\end{figure}

\begin{comment}
\underline{\textbf{Findings: }} \textit{3)} Some notable manufacturers do work hard on policy customization, but it’s difficult to improve their policy writing with the evolution of Android constantly. \textit{4)} For small and medium-sized manufacturers, little effort is paid in policy writing. \textit{5)} Even if the devices are produced by the same manufacturers in the same Android versions, their sepolicy might be different due to the customization performed by models and carriers. 
\kai{Besides the analysis of merely some numbers, more studies on details would arouse readers' interest.}
\end{comment}

\begin{summary}
  Manufacturers cannot improve their policy writing with the evolution of Android constantly, especially after the introduction of Project Treble. 
  Samsung is the only manufacturer we find that introduces self-defined attributes in policy development
  Small and medium-sized manufacturers are repeating the same mistakes made by notable manufacturers in earlier versions of Android.
  Even the same model may have different policy rules due to the customization made by carriers.
  %\kai{Besides the analysis of merely some numbers, more studies on details would arouse readers' interest.}
\end{summary}


